IntellectSeeker: A Personalized Literature Management System with the Probabilistic Model and Large Language Model

Faced with the burgeoning volume of academic literature, researchers often need help with uncertain article quality and mismatches in term searches using traditional academic engines. We introduce IntellectSeeker, an innovative and personalized intelligent academic literature management platform to address these challenges. This platform integrates a Large Language Model (LLM)--based semantic enhancement bot with a sophisticated probability model to personalize and streamline literature searches. We adopted the GPT-3.5-turbo model to transform everyday language into professional academic terms across various scenarios using multiple rounds of few-shot learning. This adaptation mainly benefits academic newcomers, effectively bridging the gap between general inquiries and academic terminology. The probabilistic model intelligently filters academic articles to align closely with the specific interests of users, which are derived from explicit needs and behavioral patterns. Moreover, IntellectSeeker incorporates an advanced recommendation system and text compression tools. These features enable intelligent article recommendations based on user interactions and present search results through concise one-line summaries and innovative word cloud visualizations, significantly enhancing research efficiency and user experience. IntellectSeeker offers academic researchers a highly customizable literature management solution with exceptional search precision and matching capabilities. The code can be found here: https://github.com/LuckyBian/ISY5001

==> result.tex <==
\section{Result}
In the IntellectSeeker system, users can browse various academic literature with unprecedented ease and precision. Users can build personalized databases through the probabilistic data capture mechanism at the platform's core. In addition, users can use the large language model in the system architecture to translate user queries into professional academic terms and optimize search efficiency. Finally, IntellectSeeker's word cloud diagram, summary summary, literature recommendation, and other functions enhance the user experience. The code can be found here: \hyperlink{https://github.com/LuckyBian/ISY5001.git}{Link}
